Optimizing Recursive Queries with Program Synthesis

Most work on query optimization has concentrated on loop-free queries. However, data science and machine learning workloads today typically involve recursive or iterative computation. In this work, we propose a novel framework for optimizing recursive queries using methods from program synthesis. In particular, we introduce a simple yet powerful optimization rule called the "FGH-rule" which aims to find a faster way to evaluate a recursive program. The solution is found by making use of powerful tools, such as a program synthesizer, an SMT-solver, and an equality saturation system. We demonstrate the strength of the optimization by showing that the FGH-rule can lead to speedups up to 4 orders of magnitude on three, already optimized Datalog systems.

==> cegis.tex <==
\section{Counterexample-guided Inductive Synthesis}\label{app:cegis}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> constraints.tex <==
\subsection{Optimization under Constraints}
Thanks to \eqsat\ and SMT-solvers,
% both stemming from automated theorem proving,
\sys\ already reasons about the semantics of the program.
It can therefore be easily extended to support semantic optimization
under constraints.

\subsubsection{Constraints in \eqsat} We extend the \eqsat-based optimization of pure
$\name$ to support constraints, by adding each constraint as a rewrite rule
for \eqsat.
In theory, any constraint $P$ can be rephrased as an equality $P = \text{true}$.
However, in order for \eqsat\ to take advantage of such general constraints,
we would have to augment the axioms to perform propositional reasoning.
Doing so essentially reinvents SMT-solvers.
Therefore in \eqsat\ we only consider any constraint that is an equality or
an implication; any implication $P_{1} \Rightarrow P_{2}$ can be rephrased as an equality $P_{1} = P_{1} \wedge P_{2}$.
For example, the invariant~\eqref{eq:invariant:tc} generates the rewrite:
%
\begin{align*}
  \bigoplus_{z} \totrop{E(x,z)} \otimes \totrop{TC(z,y)}
  =
  \bigoplus_{z} \totrop{TC(x,z)} \otimes \totrop{E(z,y)}
  \label{eq:rewrite:magic}
\end{align*}
%
where $x,y,z$ are pattern variables,
and $z_{1}, z_{2}$ from~\eqref{eq:invariant:tc} are
unified\footnote{We must unify $z_{1}, z_{2}$ to $z$
  because all pattern variables in the RHS of a rewrite rule
  must be bound in the LHS.}
to $z$.
It is easy to see how \eqsat\ can rewrite~\eqref{eq:magic:nonopt}
to~\eqref{eq:magic:opt} given the rule above.
Note this constraint is a loop invariant and is not asserted explicitly
by the user. We demonstrate in Section~\ref{sec:invariant} how to infer
such invariants automatically.

\subsubsection{Constraints and \cegis}
We support more general forms of constraints
by extending our \cegis-based synthesis procedure.
The extension is remarkably simple:
we assert all constraints every time we invoke the SMT-solver.
These assertions will lead \cegis\ to synthesize $H$ that satisfies
the constrained (therefore relaxed) FGH-rule
$\left( \bigwedge_{P \in \text{constraints}} P \right) \Rightarrow G(F(X)) = H(G(X))$.
For example, we assert~\eqref{eq:gamma:key}-\eqref{eq:gamma:neq} as well as
the invariant~\eqref{eq:invariant:tree} during synthesis to optimize~\eqref{eq:cost:nonopt}
to~\eqref{eq:cost:opt}.
% We discuss inferring~\eqref{eq:invariant:tree} in Section~\ref{sec:invariant}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> impl.tex <==
\section{Implementation}
\sys~takes as input a datalog program with two strata. The first stratum
computes an intermediate relation recursively; the second stratum takes the
intermediate and computes the output, usually with aggregation. \sys~outputs a
new datalog progam that computes the same output as the original one, given the
same input. This new program has a single stratum, and the recursion is directly
over the output relations.

\sys~simply takes the body that defines the intermediate relation as $f$; in other
words, $f$ is the immediate consequence operator in the first stratum. The second
stratum is taken as the definition of $g$. Then, \sys~tries to find $h$ such that
$h.g=g.f$, and outputs $h$ which recursively defines the output relation. Note that
in the output program, $g$ is only applied once to the program input, so the output
program need not be stratified.


Describe Rosette, EGG, \zzz.

How to encode constraints in SMT solvers.  How to enncode $\name$ programs.


==> invariant.tex <==
\subsection{Invariant Inference}\label{sec:invariant}
In Section~\ref{subsec:loop:invariants} we discussed the need for loop invariants
when applying the FGH-rule.
It is therefore desirable for the optimizer to automatically infer such invariants.
In this section we show an algorithm for invariant inference given the program
definition and integrity constraints (if any).

Recall from Corollary~\ref{cor:invariant} that an invariant $\phi$ must satisfy
$\phi(X_{0})$ and $\phi(X) \Rightarrow \phi(F(X))$.
Note $\phi(X) \Rightarrow \left(G(F(X)) =  H(G(X))\right)$ cannot be satisfied
a priori since it requires the definition of $H$;
instead, the rule is used to {\em relax} the FGH-rule and aid the synthesis of $H$.
The crucial idea of our inference algorithm is to represent an abstract domain $\Phi$ of
candidate invariants as equalities in an \egraph, and then execute $F$ {\em abstractly}
over this domain.
Any constraint satisfiying $\Phi \Rightarrow F(\Phi)$ is an invariant,
and can be found by running $F$ to a fixpoint.

We use an \egraph\ to compactly represents the constraints,
and abstractly execute $F$ on the \egraph\ to discover invariants.
We choose the initial set of candidate constraints heuristically
according to the program definition:
to the \egraph\ $\Phi_{0}$ representing the initial set
we first insert the body of each rule,
subscripting each variable $x$ and relation symbol $R$
with 0 into $x_{0}$ and $R_{0}$;
we add an equality $I_{0} = \emptyset$ for each IDB $I$,
then we run \eqsat\ using standard semiring axioms
to populate $\Phi_{0}$ with more equalities.
We execute $F$ on $\Phi_{i}$ as follows:
first we insert the rule bodies again,
this time with subscript $i+1$;
we then interpret each rule $R(a, \ldots, z) \cd e$
as a rewrite rule $R_{i+1}(a_{i+1}, \ldots, z_{i+1}) \Rightarrow e_{i}$,
where $e_{i}$ means to subscript variables and relations with $i$.
Finally we run \eqsat\ on $\Phi_{i}$ with these rules as well as the semiring axioms.
It can be shown inductively that any equality $\phi_{i+1}$ shared by $\Phi_{i}$ and $\Phi_{i+1}$ satisfies
$\forall 0 \leq j \leq i+1 . \phi_{i+1}(X_{j})$ where $X_{j}$ is the program state
at the $j$-th iteration of the concrete execution of $F$.
In other words $\phi_{i+1}$ is invariant up to the first $j$ iterations.
Therefore we only retain such $\phi_{i+1}$ in $\Phi_{i+1}$.
We repeat this until $\phi_{i}$ reaches a fixpoint, that is $\phi_{i+1} = \phi_{i}$.
At this point we have
$\left(  \bigwedge_{\phi_{i} \in \Phi_{i}} \phi_{i}(X) \right) \Rightarrow \left( \bigwedge_{\phi_{i} \in \Phi_{i}} \phi_{i}(F(X)) \right)$,
which means $\Phi_{i}$ is a loop invariant.
We can now assert all $\phi_{i} \in \Phi_{i}$ as constraints to our optimizer
for semantic optimization.

We now demonstrate the invariant inference algorithm by inferring the
invariant~\eqref{eq:invariant:tc}.
To reduce clutter, we adopt the linear algebra notation~\cite{todo}
where $ [ A \cdot B ] (x,y) = \exists z . A(x,z) \wedge B(z,y)$,
% $[A * B](x,y) = A(x,y) \wedge B(x,y)$,
and $[A + B](x,y) = A(x,y) \vee B(x,y)$.
Therefore~\eqref{eq:invariant:tc} can be rephrased as $TC \cdot E = E \cdot TC$,
and the first rule in~\eqref{eq:magic:nonopt} as $TC \cd E + TC \cdot E$.
The initial \egraph\ $\Phi_{0}$ contains, among others,
the expression $TC_{0} \cdot E$;
since every IDB implicitly starts out empty,
we add the equality $TC_{0} = \emptyset$ to $\Phi_{0}$.
Running \eqsat\ with the axiom $X \cdot \emptyset = \emptyset = \emptyset \cdot X$
leads to the equality
$TC_{0} \cdot E = \emptyset = E \cdot TC_{0}$.
So far, we have proved the invariant to hold at the initial state.
For it to be a true loop invariant, it must be {\em re-established} at
each iteration $i$. That is, $TC_{i} \cdot E = E \cdot TC_{i} \Rightarrow TC_{i+1} \cdot E = E \cdot TC_{i+1}$. The inference algorithm achieves exactly that, since we have:
\begin{align*}
  TC_{i+1} \cdot E = (E + TC_{i} \cdot E) \cdot E = (E + E \cdot TC_{i}) \cdot E & = E \cdot E + E \cdot TC_{i} \cdot E \\
  E \cdot TC_{i+1} = E \cdot (E + TC_{i} \cdot E) & = E \cdot E + E \cdot TC_{i} \cdot E
\end{align*}
where each equality follows from the property of $\cdot$ and $+$ or appplies the
constraint $TC_{i} \cdot E = E \cdot TC_{i}$, as will be deduced by \eqsat.
\remy{Remember to change the definition of $TC$ in the intro.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> semantic-opt.tex <==
\section{Equality Saturation}\label{sec:semantic-opt}

\dan{This section needs a complete rewrite.  We have very little
  space, so all we can do is to describe \eqsat\ at a high level, and
  mention that we use it in various parts of the architecture in
  Fig~\ref{fig:arch}.  GOAL: KEEP IT 1 PAGE MAX.}

\begin{figure}
  \includegraphics[width=0.45\linewidth]{egraph}
  \caption{Example \egraph.}\label{fig:eqsat}
\end{figure}

Throughout the FGH-optimizer we need to manipulate expressions, apply
rules, and manage equivalent expressions.  This problem is common to
all query optimizers.  Instead of implementing our own expression
managing model, we used a state of the art Equality Saturation
Systesm, \eqsat.  More preicsely, we used
EGG~\cite{DBLP:journals/pacmpl/WillseyNWFTP21} to implement the green
boxes in the architecture shown in Fig.~\ref{fig:arch}.

An \eqsat\ system maintains compactly a data structure called an
\egraph\ that compactly represents a set of expressions, together with
an equivalence relation over this set.  Each \egraph\ is consist of a
set of \eclasses, each \eclass\ consists of a set of \enodes, and each
\enode\ is a function symbol with \eclasses\ as children.
Figure~\ref{fig:eqsat} shows an \egraph\ representing the two
expressions in Eq.~\eqref{eq:axiom:pullmul} and their subexpressions.
The \eqsat\ system maintains separately a collection of {\em rules},
each represented by a pair of patterns.  For example, one rule may
state that $\otimes$ is commutative: $x \otimes y = y \otimes x$.  The
\eqgraph\ can efficiently add a new expression to its collection,
insert a new rule, and match a given expression against the \egraph.

We describe how we use EGG in the FGH-optimizer.  First, we use it to
extend Rule-based test (Sec.~\ref{sec:axiomatic-rewrite}) to account
for a constraint $\Gamma$.  By design, the \egraph\ makes it is easy
to infer the equivalence $p_1 = p_2$ from a set of rules.  Suppose we
want to check such an equivalence conditioned on $\Gamma$.  We assume
that $\Gamma$ is a logical implication, $\Delta \Rightarrow \Theta$.
This assumption is w.l.o.g. for our optimizer since all database
constraints are expressed this way.  We convert it into an equality
$\Delta \wedge \Theta = \Delta$, and insert it into the \egraph, then
check for equivalence $p_1=p_2$.

Second, we use the \egraph\ to denormalize an expression.  More
precisely, recall from Sec.~\ref{subsec:rule:based:synthesis} that we
attempt to synthesize $H$ by denormalizing
$p_1 \defeq \text{normalize}(F(G(X)))$, in other words, writing it in
the form $H(G(X))$.  For that we add $G(X)$ to the \egraph, observe in
which \eclass\ it is inserted, and replace that \eclass\ with a new
node $Y$.  The root of the new \egraph\ represents many equivalent
expressions, and each of them is a candidate for $H$.  We chose the
expression $H$ that has the smallest AST {\em and} does not have any
occurrence of the IDBs $X$.

Finally, we use the \egraph\ to infer the loop invariants.  We do this
by symbolically executing the recursive program $F$ for up to 4
iterations, and compute the symbolic expressions of the IDBs $X$:
$X_0, X_1, \ldots$  Using an \egraph\ we represent all identities
satisfied by these (distinct!) expressions.  The identities that are
satisfied by every $X_i$ are candidate loop invariants: for each of
them we use the SMT solver to check if they satisfy
Condition~\eqref{eq:invariant:1} (see
Sec.~\ref{subsec:loop:invariants}).








\subsubsection{Rewriting with \eqsat}
\eqsat\ can rewrite a given expression to exponentially many equivalent
expressions.
The client can then extract an expression satisfying certain properties
(in our case, matching the form $H(G(X))$)
from the results.
The central data structure of \eqsat\ is called the \egraph.
The \egraph\ 

compactly represents a set of expressions,
together with an equivalent relation over them.
Each \egraph\ is consist of many \eclasses,
each representing an equivalent class of expressions.
Each \eclass\ contains one or more \enodes,
and each \enode\ is a function symbol with \eclasses\ as children.
An \egraph\ {\em represents} an expression if any of its
\eclasses\ does; an \eclass\ represents an expression if any
of its \enodes\ does;
an \enode\ $f(c_{1}, \ldots, c_{k})$ represents
$f(e_{1}, \ldots, e_{k})$ if $c_{i}$ represents $e_{i}$ for $1 \leq i \leq k$,
and any constant \enode\ $f()$ represents $f()$.
Figure~\ref{todo} shows an \egraph\ corresponding to~\eqref{eq:axiom:pullmul}.
One expression represented is $A^{1} \otimes^{6} \bigoplus^{3}_{x^{4}} B^{2}$,
where each subexpression rooted at the symbol $\bullet^{i}$
is represented by the \eclass\ labeled with $i$.
Currently \eclass~6 represents two expressions, namely each side of~\eqref{eq:axiom:pullmul}.
Suppose we expand \eclasses~1 and 2 to include $C=A$ and $D=B$.
This doubles the sizes of \eclasses~1 and 2,
but makes \eclass~6 represent 4 times as many expressions.

To optimize a query with \eqsat, we initialize the \egraph\ by inserting
the query, creating one \eclass\ per \enode.
Then we expand the \egraph\ by adding expressions according to
a list of axioms:
we match either side of the axiom to subgraphs of the \egraph,
then insert the other side to the root \eclass\ of the matching subgraph if any.
During this process,
\eqsat\ aggressively maintains compaction by exploiting congruence and
hash-consing \enodes.\footnote{See~\cite{todo} for further details.}
We keep applying axioms until the \egraph\ stops changing,
or upon reaching a time / memory budget.
Finally, we {\em extract} one expression represented in the \egraph\
according to certain criteria,
for example to minimize a cost function or to satisfy some syntactic constraints.
As an example, we can obtain the \egraph\ in Figure~\ref{todo} as follows:
first, we create the initial \egraph\ with the left-hand-side (LHS) of~\eqref{eq:axiom:pullmul};
then we apply~\eqref{eq:axiom:pullmul}, whose LHS matches on the root of the initial \egraph;
finally we add the RHS of~\eqref{eq:axiom:pullmul} to the \egraph,
with its root \enode\ ($\bigoplus$) in the root \eclass~(6).

\subsubsection{\eqsat\ for FGH}\label{sec:eqsat:fgh}
To apply the FGH-rule with \eqsat,
we supply it with the semiring axioms,
as well as $G(F(X))$ as the input expression.
After growing the \egraph\ with the axioms,
we match $G(X)$ to subgraphs of the \egraph;
any match will give an $H$ function that makes up the rest of the \egraph\ encompassing $G(X)$.
If there are multiple matches, we use the one that results in the smallest AST for $H$.
Future work can investigate more refined cost models.

\dan{end of text that has been moved}

\input{constraints}
\input{invariant}


==> verification.tex <==
\section{Verification}

\label{sec:verification}

%%% \dan{Currently 1.5 pages.  GOAL: 1 PAGE.  Reinhard: feel free to
%%%   edit this section, hopefully shorten it.}

Given a candidate $H$, we describe here how we verify the identity
$F(G(X))=G(H(X))$, possibly in the presence of the constraint
$\Gamma$.  This step is implicit in both boxes labeled {\em Rule-based
  Synthesis} and \cegis\ in Fig~\ref{fig:arch}.

\subsection{Rule-based  Test}\label{sec:axiomatic-rewrite}
% This test consists of first normalizing both expressions, then
% checking for isomorphism.  We describe the rule-based test assuming
% there is no database constraint $\Gamma$: the extension to $\Gamma$
% can be done using a \eqsat\ system, discussed in
% Sec.~\ref{sec:semantic-opt}.


% to handle interpreted functions.
% To simplify implementation, we preprocess the input
% datalog program by mapping all semirings in the program to
% the semiring used in $G$.
% For example, the boolean semiring in $CC_{1}$ is mapped to
% the Tropical semiring as shown in Figure~\ref{fig:cc1:semiring}.
% Unifying to a single semiring saves us from enumerating
% tedious axioms describing how different semirings interact
% with each other, and also simplifies the encoding to SMT
% expressions.
% 
Let $p_{1} = G(F(X))$, $p_{2} = H(G(X))$.  To check $p_1=p_2$, the
{\em rule-based test} first normalizes both expressions into a
sum-sum-product expression (Eq.~\eqref{eq:sum:sum:product}) by
applying the semiring axioms, then checks if the expressions are
isomorphic: if yes, then $p_{1} = p_{2}$, otherwise we assume that
they are unequal.  We will discuss in Sec.~\ref{sec:semantic-opt} how
to extend this test to account for a constraint $\Gamma$.  This test
can be visualized as follows:
%
\begin{align}
  p_{1} \xrightarrow[]{\text{axioms}} \text{normalize}(p_{1})
  \simeq
  \text{normalize}(p_{2}) \xleftarrow[]{\text{axioms}} p_{2}
\label{eq:equality:isomorphism}
\end{align}
%
where $\simeq$ denotes isomorphism.  The Rule-based test is sound,
i.e. there are no false positives.  When both $p_1, p_2$ are over the
$\N^\infty$ semiring and have no interpreted functions then the test
is also
complete~\cite{DBLP:conf/icdt/Green09,DBLP:journals/pvldb/WangHSHL20}.

This simple test motivates the need for a complete set of axioms that
allows any semiring expression to be normalized.  The axioms include
standard semiring axioms, and axioms about summations and free
variable, which will play a role below.  For example, in order to
prove that $CC_1 = CC_2$ in Example~\ref{ex:fgh:cc} (shown 
% in Figures~\ref{fig:cc1} and~\ref{fig:cc2}, and
again in semiring notation in Figure~\ref{fig:cc1:semiring}) one needs
all three axioms below:
%
\begin{align}
  \bigoplus_x \bigoplus_y \left(\cdots\right) = &  \bigoplus_{x,y}\left( \cdots \right)  \label{eq:axiom:plus:plus} \\
  A \otimes \bigoplus_{x} B = & \bigoplus_{x} A \otimes B \text{ when } x \not \in \texttt{fv}(A) \label{eq:axiom:pullmul}\\
  \bigoplus_x \left(A(x) \otimes [x=y]\right) = & A(y)  \label{eq:axiom:plus:equal}
\end{align}
%

% 
% 
% 
% 
% \begin{example} We illustrate how to check of the FGH-rule in
%   Example~\ref{ex:fgh:cc}.  The two expressions $p_1, p_2$ were denote
%   $CC_1, CC_2$ and are shown in Figures~\ref{fig:cc1}
%   and~\ref{fig:cc2}.  We first de-sugar them and write them as
%   semiring expressions, as shown in Figure~\ref{fig:cc1:semiring}.
%   Recall that the cast operator $[-]_\infty^0$ maps the Boolean values
%   $0,1$ to the tropical values $\infty, 0$. We normalize both
%   expressions, using semiring axioms such as:
% %
%   \begin{align}
%     \bigoplus_x \bigoplus_y \left(\cdots\right) = &  \bigoplus_{x,y}\left( \cdots \right)  \label{eq:axiom:plus:plus} \\
%     A \otimes \bigoplus_{x} B = & \bigoplus_{x} A \otimes B \text{ when } x \not \in \texttt{fv}(A) \label{eq:axiom:pullmul}\\
%     \bigoplus_x \left(A(x) \otimes [x=y]\right) = & A(y)  \label{eq:axiom:plus:equal}
%   \end{align}
% %
%   We have designed a complete set of semiring axioms for converting
%   into a sum-sum-product expression, similar to axioms found
%   elsewhere,
%   e.g.\cite{DBLP:journals/pvldb/ChuMRCS18,DBLP:journals/pvldb/WangHSHL20}.
%   After normalization, we obtain:
% %
%   \begin{align*}
%     \text{normalize}(CC_{1}[x]) & = L[x] \oplus \bigoplus_{y,z} L[y] \otimes \totrop{E(x,z)} \otimes [TC(z,y)]_{\infty}^{0}\\
%                                 & \simeq \text{normalize}(CC_{2}[x])
%   \end{align*}
% %
%   proving their equivalence.
% %   Each rewrite step during normalization applies some semiring axioms,
% %   for example: where $\texttt{fv}(A)$ is the set of free variables in
% %   $A$.  We use standard semiring identities like the commutativity and
% %   associativity of $\oplus$ and $\otimes$ in the normalization step.
% %   We omit the exhaustive list of axioms, and refer the reader
% %   to~\cite{??} for details.
% \end{example}
% 

% In some cases this mapping is lossless;
% for example boolean disjuction $x \vee y$ can be mapped
% via inclusion-exclusion to $[x] + [y] - [x] \times [y]$,
% where $[\cdot]$ casts \texttt{true} to $1$ and
% \texttt{false} to $0$.
% In other cases this mapping is lossy.
% For example we map $\min(x,y)$ to $x+y$,
% however $\min(x,x) = x$ but $x+x \neq x$.
% In general, mapping to the sum-product semiring is always
% sound:
% \begin{theorem}[Equality over $(\N, +, \times, 0, 1)$ is canonical]\label{th:soundness}
%   $[e_{1}]_{\N} = [e_{2}]_{\N} \Rightarrow e_{1} = e_{2}$,
%   where $e_{1}$ and $e_{2}$ are over the same semiring, and
%   $[\cdot]_{\N}$ maps an expression in any semiring to the sum-product semiring.
% \end{theorem}
% We note that it is possible, albeit tedious, to skip this
% processing step and apply axioms specific to each semiring,
% and to directly encode each semiring in SMT formulas.
% An industrial-strength optimizer may opt to do so to achieve
% better coverage.
\begin{figure}
\fcolorbox{black}{light-gray}{\parbox{0.2\textwidth}{
\footnotesize
  \begin{align*}
    CC_{1}[x] & = \bigoplus_{y} L[y] \otimes \big([x=y]_{\infty}^{0} \oplus \bigoplus_{z} [E(x,z)]_{\infty}^{0} \otimes [TC(z,y)]_{\infty}^{0}\big) \\
    CC_{2}[x] & = L[x] \oplus \bigoplus_{y} \big( \bigoplus_{y'} L[y'] \otimes [TC(y,y')]_{\infty}^{0}\big) \otimes [E(x,y)]_{\infty}^{0}
  \end{align*}
}}
  \caption{$CC_{1}$ and $CC_{2}$ in semiring notation; their normal
    forms are isomorphic.}
  \label{fig:cc1:semiring}
\end{figure}
% \begin{figure}
% \fcolorbox{black}{light-gray}{\parbox{0.2\textwidth}{
% \footnotesize
%   \begin{align*}
%     CC_{2}[x] \defeq L[x] \oplus \bigoplus_{y} 1_{E(x,y)} \otimes \bigoplus_{y'} L[y'] \otimes 1_{TC(y,y')}
%   \end{align*}
% }}
%   \caption{$CC_{2}$ in semiring notation.}
%   \label{fig:cc2:semiring}
% \end{figure}

\subsection{SMT Test} \label{subsubsec:smt:test} When the
expressions $p_1, p_2$ are over a semiring other than $\N^\infty$, or
they contain interpreted functions, then the rule-based test is
insufficient.  In that case we use an SMT solver.  Modern SMT-solvers
are expressly designed to perform interpreted reasoning, and we
leverage them to extend our verifier.  We still normalize the
expressions using our axioms, because today's solvers cannot reason
about bound/free variables (as needed in
axioms~\eqref{eq:axiom:plus:plus}-\eqref{eq:axiom:plus:equal}).  The
{\em SMT test} is captured by the following figure:
% After we normalize both expressions
% $p_{1}$ and $p_{2}$, if the isomorphism test fails, then we check
% their equivalence using an SMT solver: $\Gamma \models (p_1=p_2)$.
% More precisely, we ask the solver to find a {\em counterexample}, i.e.
% IDB and EDB instances for which
% $\Gamma \wedge (\text{normalize}(p_1)\neq \text{normalize}(p_2))$.  If
% the solver fails, i.e. returns \textsf{UNSAT}, then we know that
% $p_1 = p_2$.  The following figure captures this process:
% 
% 
% If the equality is
% valid, $p_{1}$ and $p_{2}$ are equivalent; otherwise they are not, and
% the solver will return a {\em counterexample} input to $p_{1}$ and
% $p_{2}$ on which they evaluate to differnt results.  We illustrate
% this process as follows:
\begin{align}
  p_{1} \xrightarrow[]{\text{axioms}} \text{normalize}(p_{1})
  \xleftrightarrow{\text{SMT}} &
  \text{normalize}(p_{2}) \xleftarrow[]{\text{axioms}} p_{2} \label{eq:equality:smt}
\end{align}

\begin{example}[SSSP100]\label{ex:sssp100}
  Consider a labeled graph $E$ where $E[x,y]$ represents the cost of
  the edge $x,y$.  The following query computes the all-pair shortest
  path up to length of 100:
%
{\footnotesize
  \begin{align}
    D[x,y] \cd & \texttt{if } x=y \texttt{ then } 0 \texttt{ else } \min_{z} \left(D[x,z] +E[z,y]\right) \nonumber \\
    Q_{1}[x,y] \cd & \min(D[x,y],100)  \label{eq:apss:opt}
  \end{align}
}
%
  % The first rule is not {\em safe}, because $x$ does not occur in
  % relational atom; one can convert it to a safe rule by restricting
  % $x$ to range over the set of nodes in the graph, but we omit that in
  % order to reduce clutter.  The second rule is both recursive {\em
  %   and} contains an aggregate operator, $\min$.  If one were to
  % represent it in standard datalog, it would be something like this:
%
  % \begin{align*}
  %   D(x,y,\min(v+c)) \cd & D(x,z,v),E(z,y,c)
  % \end{align*}
%
  % In standard datalog rules with aggregates are not monotone.  In
  % order to add such rules to datalog, prior
  % work~\cite{DBLP:conf/pods/GangulyGZ91,DBLP:journals/tkde/SeoGL15}
  % has re-defined the semantics of the $\min$ operator, whenever it
  % occurs in the head of a recursive rule.  Instead, in $\name$ our
  % approach is to use a standard semantics, by generalizing from the
  % Boolean semiring to an arbitrary ordered semiring.  The
  % program~\eqref{eq:apss:opt} is interpreted over the tropical
  % semiring $\trop = (\N \cup \set{\infty},\min,+,\infty,0)$.  The
  % program is monotone and has a unique least fixpoint.
  The program is inefficient because it first computes the full path
  length, only to cap it later to 100.  By using the FGH-rule we can
  optimize it to:
%
{\footnotesize
  \begin{align}
    Q_{2}[x,y] \cd & \texttt{if } x=y \texttt{ then } 0 \texttt{ else } \min\left(\min_{z} \left(Q_{2}[x,z]+E[z,y]\right),100\right) \label{eq:apss:opt:opt}
  \end{align}
}
%
Both are programs over the tropical semiring. We show how to verify
that~\eqref{eq:apss:opt:opt} is equivalent to~\eqref{eq:apss:opt}.
Denote by $P_1 \defeq G(F(D))$ and $P_2 \defeq H(G(D))$ (where $F,G,H$
are the obvious functions in the programs $Q_1, Q_2$).  After we
de-sugar, convert them to semring expressions, and normalize them,
they become:
%
{\footnotesize
\begin{align*}
  P_{1}[x,y] & =  \left(0 \otimes \totrop{x=y}\right) \oplus \left(\bigoplus_{z} D[x,z] \otimes E[z,y]\right)\oplus 100 \\
  P_{2}[x,y] % & = 0 \otimes \totrop{x=y} \oplus 100 \oplus \bigoplus_{z} (D[x,z] \oplus 100) \otimes E[z,y] \\
             % & = 0 \otimes \totrop{x=y} \oplus 100 \oplus \bigoplus_{z} D[x,z] \otimes E[z,y] \\
             % & \hskip 59pt \oplus \bigoplus_{z} 100 \otimes E[z,y] \\
%              & = 100 \oplus 0 \otimes \totrop{x=y} \oplus \bigoplus_{z} D[x,z] \otimes E[z,y] \\
%              & \hskip 25pt \oplus 100 \otimes \bigoplus_{z} E[z,y] \\
             & = \left(0 \otimes \totrop{x=y}\right) \oplus \left(\bigoplus_{z} D[x,z] \otimes E[z,y]\right)  \oplus \left(100 \otimes\bigoplus_{z} E[z,y]\right)\oplus 100
\end{align*}
}
%
In the normalized expressions we push the summations past the joins,
i.e. we apply rule~\eqref{eq:axiom:pullmul} from right to left, thus
we write $100 \otimes \bigoplus (\cdots)$ instead of
$\bigoplus (100 \otimes \cdots)$: we give the rationale below.  At
this point, the normalized $P_{1}$ and $P_{2}$ are not isomorphic, yet
they are equivalent if they are interpreted in the tropical semiring.
We explain below in detail how the solver can check that. Here we give
a short argument, by noting that, in this particular semiring the
following identity holds:
\[
  100 = \left(100 \otimes \bigoplus_{z} E[z,y]\right)  \oplus 100
\]
This is immediately seen once we replace the uninterpreted operators
$\oplus, \otimes$ with $\min, +$, and obtain this identity for
$E[z,y] \geq 0$:
%
\begin{align}
& 100 = \min(100 + \min_{z} E[z,y],100) \label{eq:min100}
\end{align}
%
% As we explain below, an SMT solver can prove this identity given that
% $E[z,y] \geq 0$.  More precisely, using the \zzz\ solver, we discover
% that the following is \textsf{UNSAT}:
% \[
% x \geq 0 \wedge 100 \neq \min(100 + x, 100)
% \]
% from which we can conclude
% $\forall x . x \geq 0 \Rightarrow 100 = \min(100, 100 + x)$.
\end{example}


We describe now how we implemented the SMT-test
$\Gamma \models p_1 = p_2$ using a solver.  Recall that $\Gamma$ is
the database constraint, and $p_1, p_2$ are the expressions $G\circ F$
and $H \circ G$. We used the \zzz\ solver in our system, but our
discussion applies to other solvers as well. We need to normalize
$p_1, p_2$ before using the solver, because solvers require all axioms
to be expressed in First Order Logic, and cannot encode the
axioms~\eqref{eq:axiom:plus:plus}-\eqref{eq:axiom:plus:equal}, because
they are referring to free variables in expressions, which is a
meta-logical condition, and not expressible in First Order Logic.
Once normalized, we encode the equality as a first-order logic
formula, and assert its negation, asking the solver to check if
$\Gamma \wedge \left(p_1 \neq p_2\right)$ is satisfiable.  The solver
can return one of three values: $\textsf{UNSAT}$, a counterexample, or
$\textsf{UNKNOWN}$.  When it returns $\textsf{UNSAT}$, then the
identity holds.  When it returns a counterexample, then the identity
fails, and the counterexample is given as input to the synthesizer
(Sec.~\ref{subsec:synthesis}).  $\textsf{UNKNOWN}$ means that it could
neither prove nor disprove the equivalence: this happens when the
theory is undecidable~\cite{DBLP:conf/cav/GeM09}, and in that case we
simply assume that $p_1 \neq p_2$.  The theory of reals with $+, *$ is
decidable, by Tarski's theorem, but its complexity is
hyper-exponential and \zzz\ often timed out in our experiments.
Instead, we used the theory of integers with $+, *$.  Although this
theory is undecidable, \zzz\ solved all our examples quickly, and
never returned $\textsf{UNKNOWN}$.  We encode every $\bm S$-relation
$R(x_1, \dots, x_n)$ as an uninterpreted function
$R : \N \times \cdots \times \N \rightarrow \bm S$, where $\bm S$ is
the {\em interpreted} semiring, i.e. Booleans, or the tropical
semiring, or $\N^\infty$ etc.  We represent natural numbers as
integers plus the assertion that they are nonnegative, and represent
the sets $\N^\infty, \N_\bot, \R_\bot$ union types.  For every
operator, if it is one supported by the solver, like $+, *, \min, -$,
then we entered into the formula unchanged, otherwise we treat it as
an uninterpreted function.  Unbounded aggregation, like
$\bigoplus_{x} e(x)$, poses a challenge, since there is no
corresponding operation in any SMT theory.
%%% One may attempt to unfold
%%% the aggregate over some bounded values of $x$, say replace
%%% $\min_{x} e(x)$ with $\min(e(0), \dots, e(20))$, but this approach is
%%% unsound.
Our solution uses the fact that both $p_1$ and $p_2$ are normalized
sum-sum-product expressions:
%
\begin{align*}
p_1 = & \left(\bigoplus_{x_1} e_1\right) \oplus \left(\bigoplus_{x_2}  e_2\right) \oplus \cdots 
& 
p_2 = & \left(\bigoplus_{x_1'} e_1'\right) \oplus \left(\bigoplus_{x_2'} e_2'\right) \oplus \cdots
\end{align*}
%
Assume first that each $x_i$ is a single variables. We start by
ensuring that all the variables $x_1, x_2, \ldots$ in $p_1$ are
distinct, by renaming them if necessary.  Next, we replace each
expression $\bigoplus_{x_i} e_i$ with $u(x_i,e_i)$ where $u$ is an
uninterpreted function.  Finally, we ask the solver to check whether
%
\begin{align}
\Gamma \models \left(u(x_1,e_1) \oplus u(x_2,e_2) \oplus \cdots =  u(x_1',e_1') \oplus u(x_2',e_2') \oplus \cdots\right) \label{eq:ui:uj}
\end{align}
%
This procedure is sound, because if the identity $u(x,e) = u(x',e')$
holds, then $x=x'$ (they are the same variable) and $e=e'$, which
means that $\bigoplus_x e = \bigoplus_{x'} e'$.  The procedure is also
complete in a limited sense.  Since $p_2$ is synthesized, we will
ensure that the generator includes the variables $x_1, x_2, \ldots$
present in $p_1$ when generating the summations $p_2$, see
Sec.~\ref{subsec:synthesis}; if a right correspondence between the
variables exists, then the synthesizer will find it.  Finally, if a
summation is over multiple variables, we simply nest the uninterpreted
function, i.e. write $\bigoplus_{x,y} e$ as $u(x,u(y,e))$.

\begin{example}  We finish Example~\ref{ex:sssp100} by showing how the
  solver can check that $P_1 = P_2$.  After introducing the
  uninterpreted functions described above, we obtain:
%
  \begin{align*}
    P_1 = & \min(0+w(x,y), u(z,D[x,z]+E[z,y]), 100) \\
    P_2 = & \min(0+w(x,y), u(z,D[x,z]+E[z,y]), 100+u(z,E[z,y]), 100)
  \end{align*}
  where $w(x,y)$ is an uninterpreted function representing
  $[x=y]_\infty^0$, and $u$ is our uninterpreted function encoding
  summation.  The solver proves that the two expressions are equal,
  given that $w \geq 0$ and $u \geq 0$.  Notice that it was critical
  to factorize the term 100: had we not done that, then the expression
  $100+u(z,E[z,y])$ would be $u(z,100 + E[z,y])$ and the identity
  $P_1=P_2$ no longer holds.
\end{example}

\reinhard{uniform notation: $p_1$ and $p_2$ vs. $P_1$ and $P_2$?}


% This encoding of aggregates is complete
% in the following sense:
% %
% \begin{theorem}[Encoding $\bigoplus$ with uninterpreted functions]
%   $\bigoplus_{x} e = \bigoplus_{x'} e' \Leftrightarrow f_{\bigoplus}(x, e) = f_{\bigoplus}(x',e')$
%   where $\bigoplus_{x} e$ and $\bigoplus_{x'} e'$ are in normal form.
% \end{theorem}
% %
% The following shows the SMT encoding of $Q_{1}$ and $Q_{2}$:
% \begin{align*}
%   Q_{1} & : \min(100, 0 + \totrop{x=y}, f_{\min}(z, f_{D}(x,z) + f_{E}[z,y])) \\
%   Q_{2} & : \min(100, 0 + \totrop{x=y}, f_{\min}(z, f_{D}(x,z) + f_{E}[z,y]), \\
%         & \hskip 26pt 100 + f_{\min}(z, f_{E}[z,y]))
% \end{align*}

%%% \subsubsection{Discussion} In summary, our verifier checks $p_1 = p_2$
%%% by first normalizing both expressions, checking for isomorphism,
%%% \eqref{eq:equality:isomorphism} and, if that fails, then using the
%%% \zzz\ solver to check their equivalence, \eqref{eq:equality:smt}.  The
%%% reader may wonder why we don't bypass normalization altogether and
%%% perform the entire verification pipeline in the solver.  The reason is
%%% that the solver requires all axioms to be expressed in First Order
%%% Logic, while some crucial axioms needed for identities of
%%% sum-sum-product expressions require checking for free variables, as in
%%% example~\eqref{eq:axiom:pullmul}, which is a meta-logical condition,
%%% and not expressible in First Order Logic.  In other words, we are
%%% extending the solver with specialized knowledge about the semiring.

% 
% Moreover, other axioms
% expressible in FOL usually require quantification and can easily make
% SMT-solving undecidable or intractable. \dan{I don't understand the
%   last sentence}

% In summary, the verification process first normalizes the pair of expressions
% to be checked.
% If the normal forms are isomorphic, the expressions are equivalent and verification succeeds.
% Otherwise, we encode the expressions in an SMT formula that asserts their equivalence,
% then checks the validity of this formula with an SMT sovler.
% The entire pipeline looks like the following:

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

